Criss-Cross Insertion and Deletion Correcting Codes

This paper studies the problem of constructing codes correcting deletions in arrays. Under this model, it is assumed that an $n\times n$ array can experience deletions of rows and columns. These deletion errors are referred to as $(t_r,t_c)$-criss-cross deletions if $t_r$ rows and $t_c$ columns are deleted, while a code correcting these deletion patterns is called a $(t_r,t_c)$-criss-cross deletion correction code. The definitions for criss-cross insertions are similar. It is first shown that when $t_r=t_c$ the problems of correcting criss-cross deletions and criss-cross insertions are equivalent. The focus of this paper lies on the case of $(1,1)$-criss-cross deletions. A non-asymptotic upper bound on the cardinality of $(1,1)$-criss-cross deletion correction codes is shown which assures that the redundancy is at least $2n-3+2\log n$ bits. A code construction with an existential encoding and an explicit decoding algorithm is presented. The redundancy of the construction is at most $2n+4 \log n + 7 +2 \log e$. A construction with explicit encoder and decoder is presented. The explicit encoder adds an extra $5\log n + 5$ bits of redundancy to the construction.

==> decoder.tex <==
\begin{itemize}
	\item If equivalence of insertion and deletions holds is there also insertion decoder?
\end{itemize}

==> problems.tex <==
Problems to look at: \begin{enumerate}
    \item Decoder for single insertion (same construction holds)
    \textcolor{green!50!black}{Hopefully done.}
    \item Insertions: regular size? is there an expression? \textcolor{red}{Insertion ball is not regular, working on several directions here.} \textcolor{green!50!black}{Left as a future direction, if needed.}
    \item Nice non-asymptotic bound
    \textcolor{green!50!black}{Hopefully done.}
    \item Explicit {\em encoder} for the insertion/deletion correction construction.
    \textcolor{green!50!black}{Hopefully done}
    % \item Non binary setting (our construction and bounds should hold, maybe this setting is not that important)
    % \item Exact ball size for deletions (HARD)
\end{enumerate}

\noindent {\bf Other paper:} \begin{enumerate}    
    \item Improving the redundancy of the current construction? (HARD)
    \item Generalized Criss-Cross deletions/insertions: bounds and constructions using Gabidulin codes
    \item Multiple deletions (construction plus bound). Start with burst deletions
    \item Multiple insertions. Start with burst
    \item $3$-dimensional arrays?? (educated guess: construction could be extended if deletions are planes)
    \item Combinations of insertions and deletions, e.g., one inserted row and one deleted column
\end{enumerate}

==> qary.tex <==
Extension for q-ary alphabet
